Mitigating Source Bias for Fairer Weak Supervision

Weak supervision enables efficient development of training sets by reducing the need for ground truth labels. However, the techniques that make weak supervision attractive -- such as integrating any source of signal to estimate unknown labels -- also entail the danger that the produced pseudolabels are highly biased. Surprisingly, given everyday use and the potential for increased bias, weak supervision has not been studied from the point of view of fairness. We begin such a study, starting with the observation that even when a fair model can be built from a dataset with access to ground-truth labels, the corresponding dataset labeled via weak supervision can be arbitrarily unfair. To address this, we propose and empirically validate a model for source unfairness in weak supervision, then introduce a simple counterfactual fairness-based technique that can mitigate these biases. Theoretically, we show that it is possible for our approach to simultaneously improve both accuracy and fairness -- in contrast to standard fairness approaches that suffer from tradeoffs. Empirically, we show that our technique improves accuracy on weak supervision baselines by as much as 32\% while reducing demographic parity gap by 82.5\%. A simple extension of our method aimed at maximizing performance produces state-of-the-art performance in five out of ten datasets in the WRENCH benchmark.

==> rebuttal/rebuttal_one_pager.tex <==
\newpage
\setcounter{figure}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}

\section{Rebuttal Supplementary Materials}
\subsection{Experiment on the number of LFs}
\begin{figure}[h]\small
\small
	\centering
	\subfigure [Number of LFs vs. Performance]{
\includegraphics[width=0.49\textwidth]{rebuttal/synthetic_LF_num_lfs_performance.pdf}}
\subfigure [Number of LFs vs. Unfairness]{
\includegraphics[width=0.49\textwidth]{rebuttal/synthetic_LF_num_lfs_fairness.pdf}}
\caption{Synthetic experiment on number of LFs vs. performance and fairness. Labeling functions are generated by sampling centers $x^{center_j}$ and scaling parameters $\theta_j$. \textbf{The result shows that simply diversifying label sources does not improve fairness---though performance can be improved by adding more LFs. On the other hand, SBM resolves unfairness and yields better performance by mitigating source bias.} Here, $n=10000$ input samples in $\real^{2}$ are taken from $\sim \mathcal{N}(0, I)$, and true labels $Y$ are generated by $Y = 1[X[:, 0] \geq 0]$. Group transformation   $g_b(x): x+b$ is applied to a random half of samples, where $b \sim \mathcal{U}([10, 50]^2)$. Parameters for each LFs are sampled from $\theta_j \sim \mathcal{U}(0.1, 3)$, $x^{center_j} \sim \mathcal{U}([-5, 5]^2)$.}
\label{fig:rebuttal_num_lfs}
\vspace{-5mm}
\end{figure}

\subsection{Experiment results with error ranges}
We report results with error ranges. Here we provide Figure 4 (synthetic experiment results) with confidence intervals. \textbf{In addition, real data experimental result tables with standard deviations are included on the rebuttal page}. We will include both in our updated manuscript.

\begin{figure}[h]\small
\small
	\centering
	\subfigure [Number of samples vs. Performance]{
\includegraphics[width=0.49\textwidth]{rebuttal/synthetic_LF_performance.pdf}}
\subfigure [Number of samples vs. Unfairness]{
\includegraphics[width=0.49\textwidth]{rebuttal/synthetic_LF_fairness.pdf}}
\caption{Synthetic experiment on number of samples vs. performance and fairness. Confidence intervals are obtained by $\pm 1.96 \times $ standard deviation of 10 repetition with different seeds. \textbf{We  observe that SBM obtains the counterfactual mapping efficiently, improving performance and fairness at the same time. Meanwhile, performance and fairness of vanilla WS cannot be improved by increasing the  number of samples due to bias.}}
\label{fig:rebuttal_num_samples}
\vspace{-5mm}
\end{figure}

